R\'egularisation et optimisation pour l'imagerie sismique des fondations de pyl\^ones

This research report summarizes the progress of work carried out jointly by the IRCCyN and the \'Ecole Polytechnique de Montr\'eal about the resolution of the inverse problem for the seismic imaging of transmission overhead line structure foundations. Several methods aimed at mapping the underground medium are considered. More particularly, we focus on methods based on a bilinear formulation of the forward problem on one hand (CSI, modified gradient, etc.) and on methods based on a "primal" formulation on the other hand. The performances of these methods are compared using synthetic data. This work was partially funded by RTE (R\'eseau de Transport d'\'Electricit\'e), which has initiated the project, and was carried out in collaboration with EDF R&D (\'Electricit\'e de France - Recherche et D\'eveloppement).

==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath et bm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}

%%%% NEW - NEW - %%%%% Small caps gras %%%% 05-06-98 %%%% JFG %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Merci \`a Caro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareFontShape{T1}{cmr}{bx}{sc}{
         <8> <9> <10> <10.95> dcbsc10
         <12> <14.4> dcbsc10
         <17.28> <20.74> <24.88> dcbsc10
         }{}
% SC en bold (Hack !)
\DeclareFontShape{T1}{cmr}{b}{sc}{
         <8> <9> <10> <10.95> dcbsc10
         <12> <14.4> dcbsc10
         <17.28> <20.74> <24.88> dcbsc10
         }{}%

\def\scb#1{\bfseries {\scshape #1}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% DEFINITIONS PRELIMINAIRES 

% definition pour \xspace
\def\XS{\xspace}

% Style gras italique (Necessite amsmath)
\def\sbm#1{\ensuremath{\bm{#1}}}               
%% \DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
%% \def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique

% Style droit en math
\def\sdm#1{\ensuremath{\mathrm{#1}}}

% Style gras droit
\def\sbv#1{\ensuremath{\mathbf{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ALPHABET GRAS ITALIQUE
% Taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% ALPHABET CURSIF
% Cursif(majuscules), taille adaptative

\def\Ac{{\ensuremath{\mathcal{A}}}\XS}
\def\Bc{{\ensuremath{\mathcal{B}}}\XS}
\def\Cc{{\ensuremath{\mathcal{C}}}\XS}
\def\Dc{{\ensuremath{\mathcal{D}}}\XS}
\def\Ec{{\ensuremath{\mathcal{E}}}\XS}
\def\Fc{{\ensuremath{\mathcal{F}}}\XS}
\def\Gc{{\ensuremath{\mathcal{G}}}\XS}
\def\Hc{{\ensuremath{\mathcal{H}}}\XS}
\def\Ic{{\ensuremath{\mathcal{I}}}\XS}
\def\Jc{{\ensuremath{\mathcal{J}}}\XS}
\def\Kc{{\ensuremath{\mathcal{K}}}\XS}
\def\Lc{{\ensuremath{\mathcal{L}}}\XS}
\def\Mc{{\ensuremath{\mathcal{M}}}\XS}
\def\Nc{{\ensuremath{\mathcal{N}}}\XS}
\def\Oc{{\ensuremath{\mathcal{O}}}\XS}
\def\Pc{{\ensuremath{\mathcal{P}}}\XS}
\def\Qc{{\ensuremath{\mathcal{Q}}}\XS}
\def\Rc{{\ensuremath{\mathcal{R}}}\XS}
\def\Sc{{\ensuremath{\mathcal{S}}}\XS}
\def\Tc{{\ensuremath{\mathcal{T}}}\XS}
\def\Uc{{\ensuremath{\mathcal{U}}}\XS}
\def\Vc{{\ensuremath{\mathcal{V}}}\XS}
\def\Wc{{\ensuremath{\mathcal{W}}}\XS}
\def\Xc{{\ensuremath{\mathcal{X}}}\XS}
\def\Yc{{\ensuremath{\mathcal{Y}}}\XS}
\def\Zc{{\ensuremath{\mathcal{Z}}}\XS}

% Lettres cursives grasses (majuscules)
%
\def\Acb{{\sbm{\mathcal{A}}}\XS}
\def\Bcb{{\sbm{\mathcal{B}}}\XS}
\def\Ccb{{\sbm{\mathcal{C}}}\XS}
\def\Dcb{{\sbm{\mathcal{D}}}\XS}
\def\Ecb{{\sbm{\mathcal{E}}}\XS}
\def\Fcb{{\sbm{\mathcal{F}}}\XS}
\def\Gcb{{\sbm{\mathcal{G}}}\XS}
\def\Hcb{{\sbm{\mathcal{H}}}\XS}
\def\Icb{{\sbm{\mathcal{I}}}\XS}
\def\Jcb{{\sbm{\mathcal{J}}}\XS}
\def\Kcb{{\sbm{\mathcal{K}}}\XS}
\def\Lcb{{\sbm{\mathcal{L}}}\XS}
\def\Mcb{{\sbm{\mathcal{M}}}\XS}
\def\Ncb{{\sbm{\mathcal{N}}}\XS}
\def\Ocb{{\sbm{\mathcal{O}}}\XS}
\def\Pcb{{\sbm{\mathcal{P}}}\XS}
\def\Qcb{{\sbm{\mathcal{Q}}}\XS}
\def\Rcb{{\sbm{\mathcal{R}}}\XS}
\def\Scb{{\sbm{\mathcal{S}}}\XS}
\def\Tcb{{\sbm{\mathcal{T}}}\XS}
\def\Ucb{{\sbm{\mathcal{U}}}\XS}
\def\Vcb{{\sbm{\mathcal{V}}}\XS}
\def\Wcb{{\sbm{\mathcal{W}}}\XS}
\def\Xcb{{\sbm{\mathcal{X}}}\XS}
\def\Ycb{{\sbm{\mathcal{Y}}}\XS}
\def\Zcb{{\sbm{\mathcal{Z}}}\XS}


% ALPHABET DROIT EN MATHS
% Taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT
% Permet d'obtenir des caracteres droits directement 
% en mode math ou pas math.
% (Un peu moins utile peut \^eetre)

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% ALPHABET GREC GRAS 
% Enrichie, completee et modifi\'ee par J.-F. Gio.
% Taille adaptative !

\def\alphab      {{\sbm{\alpha}}\XS}
\def\betab       {{\sbm{\beta}}\XS}
\def\gammab      {{\sbm{\gamma}}\XS}      \def\Gammab    {{\sbm{\Gamma}}\XS}
\def\deltab      {{\sbm{\delta}}\XS}      \def\Deltab    {{\sbm{\Delta}}\XS}
\def\epsilonb    {{\sbm{\epsilon}}\XS}
\def\varepsilonb {{\sbm{\varepsilon}}\XS}
\def\etab        {{\sbm{\eta}}\XS}
\def\thetab      {{\sbm{\theta}}\XS}      \def\Thetab    {{\sbm{\Theta}}\XS}
\def\varthetab   {{\sbm{\vartheta}}\XS}
\def\iotab       {{\sbm{\iota}}\XS}
\def\kappab      {{\sbm{\kappa}}\XS}
\def\lambdab     {{\sbm{\lambda}}\XS}    \def\Lambdab   {{\sbm{\Lambda}}\XS}
\def\mub         {{\sbm{\mu}}\XS}
\def\nub         {{\sbm{\nu}}\XS}
\def\xib         {{\sbm{\xi}}\XS}                 \def\Xib        {{\sbm{\Xi}}\XS}
\def\pib         {{\sbm{\pi}}\XS}                 \def\Pib        {{\sbm{\Pi}}\XS}
\def\varpib      {{\sbm{\varpi}}\XS}
\def\rhob        {{\sbm{\rho}}\XS}
\def\varrhob     {{\sbm{\varrho}}\XS}
\def\sigmab      {{\sbm{\sigma}}\XS}      \def\Sigmab    {{\sbm{\Sigma}}\XS}
\def\varsigmab   {{\sbm{\varsigma}}\XS}  \def\Varsigmab {{\sbm{\Varsigma}}\XS}
\def\phib        {{\sbm{\phi}}\XS}        \def\Phib       {{\sbm{\Phi}}\XS}
\def\varphib     {{\sbm{\varphi}}\XS}
\def\chib        {{\sbm{\chi}}\XS}
\def\psib        {{\sbm{\psi}}\XS}        \def\Psib       {{\sbm{\Psi}}\XS}
\def\omegab      {{\sbm{\omega}}\XS}      \def\Omegab    {{\sbm{\Omega}}\XS}
\def\taub        {{\sbm{\tau}}\XS}
\def\upsilonb    {{\sbm{\upsilon}}\XS}   \def\Upsilonb  {{\sbm{\Upsilon}}\XS}
\def\zetab       {{\sbm{\zeta}}\XS}


% CHIFFRES
% Gras, taille adaptative

\def\zerob       {{\sbv{0}}\XS}
\def\unb                 {{\sbv{1}}\XS}
\def\deuxb       {{\sbv{2}}\XS}
\def\troisb      {{\sbv{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}
\def\cinqb       {{\sbv{5}}\XS}
\def\sixb        {{\sbv{6}}\XS}
\def\septb       {{\sbv{7}}\XS}
\def\huitb       {{\sbv{8}}\XS}
\def\neufb       {{\sbv{9}}\XS}


% QUELQUES ENSEMBLES
% Taille adaptative

\def\eC{{\ensuremath{\mathbb C}}\XS}
\def\eE{{\ensuremath{\mathbb E}}\XS}
\def\eN{{\ensuremath{\mathbb N}}\XS}
\def\eR{{\ensuremath{\mathbb R}}\XS}
\def\eZ{{\ensuremath{\mathbb Z}}\XS}
\def\eC{{\ensuremath{\mathbb C}}\XS}

